Magnetic fields from low mass stars to brown dwarfs

Magnetic fields have been detected on stars across the H-R diagram and substellar objects either directly by their effect on the formation of spectral lines, or through the activity phenomena they power which can be observed across a large part of the electromagnetic spectrum. Stars show a very wide variety of magnetic properties in terms of strength, geometry or variability. Cool stars generate their magnetic fields by dynamo effect, and their properties appear to correlate - to some extent - with stellar parameters such as mass, rotation and age. With the improvements of instrumentation and data analysis techniques, magnetic fields can now be detected and studied down to the domain of very-low-mass stars and brown dwarfs, triggering new theoretical works aimed, in particular, at modelling dynamo action in these objects. After a brief discussion on the importance of magnetic field in stellar physics, the basics of dynamo theory and magnetic field measurements are presented. The main results stemming from observational and theoretical studies of magnetism are then detailed in two parts: the fully-convective transition, and the very-low mass stars and brown dwarfs domain.

==> pst/zeeman-pol.tex <==
\begin{pspicture}(0,0)(\textwidth,-9)
  % repère
  \psline[linecolor=gray]{->}(7,-8)(7,-1) % axe z
  \rput(7.5, -1){$z$}
  \psline[linecolor=gray]{->}(7,-5)(12,-5) % axe y
  \rput(12, -4.5){$y$}
  \psline[linecolor=gray]{->}(7,-5)(3.5,-7) % axe x
  \rput(3, -7){$x$}
  % vecteur B
  \psline[linewidth=2pt]{->}(7,-5)(7,-3.5)
  \rput(7.5,-4){$\vec{B}$}
  % polarisation circulaire sur l'axe z
  \psellipse(7,-2)(1,0.2) \psline[linewidth=2pt]{->}(7,-2.2)(6.99,-2.2)
  \rput(8.5,-2){$\sigma_r$}
  \psellipse(7,-2.8)(1,0.2) \psline[linewidth=2pt]{->}(7,-3)(7.01,-3)
  \rput(8.5,-3){$\sigma_b$}
  \psellipse(7,-6.5)(1,0.2) \psline[linewidth=2pt]{->}(7,-6.7)(7.01,-6.7)
  \rput(8.5,-6.5){$\sigma_b$}
  \psellipse(7,-7.3)(1,0.2) \psline[linewidth=2pt]{->}(7,-7.5)(6.99,-7.5)
  \rput(8.5,-7.5){$\sigma_r$}
  % polarisation linéaire sur l'axe x
  \psline(3.4,-6.7)(4.5,-6.7) \rput(3.5,-6.5){$\sigma_b$}
  \psline(4.6,-5.9)(4.6,-6.9) \rput(4.4,-6.3){$\pi$}
  \psline(4.7,-6)(5.8,-6) \rput(4.9,-5.8){$\sigma_r$}
  % polarisation linéaire sur l'axe y
  \psline(10.6,-5.2)(11.4,-4.8) \rput(11,-4.5){$\sigma_r$}
  \psline(10.4,-5.4)(10.4,-4.6) \rput(10.4,-4.4){$\pi$}
  \psline(9.4,-5.2)(10.2,-4.8) \rput(9.8,-4.5){$\sigma_b$}
\end{pspicture}
